Instrument-To-Instrument translation: Instrumental advances drive restoration of solar observation series via deep learning

The constant improvement of astronomical instrumentation provides the foundation for scientific discoveries. In general, these improvements have only implications forward in time, while previous observations do not benefit from this trend. Here we provide a general deep learning method that translates between image domains of different instruments (Instrument-To-Instrument translation; ITI). We demonstrate that the available data sets can directly profit from the most recent instrumental improvements, by applying our method to five different applications of ground- and space-based solar observations. We obtain 1) solar full-disk observations with unprecedented spatial resolution, 2) a homogeneous data series of 24 years of space-based observations of the solar EUV corona and magnetic field, 3) real-time mitigation of atmospheric degradations in ground-based observations, 4) a uniform series of ground-based H$\alpha$ observations starting from 1973, 5) magnetic field estimates from the solar far-side based on EUV imagery. The direct comparison to simultaneous high-quality observations shows that our method produces images that are perceptually similar and match the reference image distribution.

==> sections/discussion_addition.tex <==
% \section{Discussion}

% interpretation of training - advantages over paired training
%The learning with unpaired samples allows the use of real observations as reference image. This provides a natural upper limit of image enhancement and avoids artificial assumptions about the mapping between high- and low-quality observations. This is in contrast to image enhancement with paired samples, where assumptions are required to provide a high-quality reference. Furthermore, the diversity of synthetic low-quality samples allows our model to recover a broad set of degradations from real low-quality observations, as can be seen from Sect.~\ref{section:iti_diversity} and \ref{section:iti_restoration}, where our method strongly reduced the impact of clouds in H$\alpha$ full-disk observations. The adversarial training of our method ensures that translated images correspond to the real image domains. Hereby the discriminator A ensures the generation of realistic low-quality observations, which improves the applicability to real observations. While discriminator B enforces that enhanced observations show high-quality characteristics, which restricts the number of possible solutions for image enhancement and increases the perceptual quality.

% discussion (maybe):  recover overexposed regions \citep{}.

% results of enhancement
%From all the considered instrument translations a strong increase in image quality can be observed in the form of sharpening of solar structures, corrections of saturated regions, contrast enhancement and mitigation of atmospheric effects (Sect.~\ref{section:iti_restoration} and \ref{section:iti_atmospheric}). The training with image patches allows the enhancement of full-disk images in the highest resolution. Our method shows a strong enhancement of small-scale structures (Sect.~\ref{section:iti_multi}, \ref{section:iti_fov}), while the enhancement is consistent over large scales. Thus, the neural network shows strong enhancement performance independent of the spatial location on the solar disk and also large-scale solar features are preserved in their appearance. The images are normalized by a fixed value range as estimated from the full data set, which makes the intensity scaling instrument specific. Our method provides a photometric adjustment and homogenization of instrumental characteristics, which is essential for long-term (solar cycle) studies that need to a) combine  different instruments (cross-calibration) and b) need to account for instrument degradation over its life-time (calibration). This can be seen from enhanced EUV observations from SOHO/EIT that were adjusted to the intensity distribution of the SDO/AIA EUV filtergrams, as can be seen from the comparison of full-disk images (Fig.~\ref{figure:soho_sdo_full}) and the comparison of light-curves derived from the image series (Fig.~\ref{figure:soho_sdo_lightcurve}). Similarly photographic film was reconstructed to CCD quality by mitigation of saturation and adjustment of global illumination (Sect.~\ref{section:iti_restoration}).

% evaluation
%All of the considered data sets have a very small or no temporal overlap of observations. This has two implications for the obtained results. On the one hand, the neural network was never trained with real paired images. The obtained results are therefore not obtained from memorization. The use of unpaired samples typically allows for the use of larger data sets which counteracts the appearance of artifacts and mode collapse. On the other hand, the absence of paired samples makes the evaluation, and therefore the assessment of reliability, more difficult. For all applications in Sect.~\ref{section:iti_results} we selected random samples from the data set, that serve for a qualitative comparison. The comparison of light-curves demonstrates the correct adjustment of the intensity distribution between instruments (Sect.~\ref{section:iti_multi}). The overlap between the considered data sets is sparse, but we note that the pixel-wise comparison of these pairs might provide an additional estimate of the performance of our approach.

% usefulness of the provided data
%For all the considered data sets the enhanced observations show a strong similarity to the corresponding high-quality images. The comparison of SOHO and SDO light-curves suggest that our method provides a correct instrumental adjustment over long time periods. This allows the homogenization of data sets for the analysis of legacy data and study of solar cycle variations \citep[cf.][]{chatzistergos2019analysis, hamada2020new}. This calibration also applies to applications with no direct overlap, like STEREO-to-SDO, that provide unified observation of the Sun from multiple viewpoints. The direct comparison with real observations from Hinode (Fig.~\ref{figure:hmi_hinode} and \ref{figure:hmi_hinode_samples}) suggest that solar features are correctly mapped into the high-quality domain. These results demonstrate that our method provides a suitable addition to the study of the solar surface in high resolution, e.g. as context information from adjacent regions. Our methods shows the ability to mitigate multiple atmospheric influences simultaneously, leading to a more stable observations series in the highest quality (Sect.~\ref{section:iti_atmospheric}). This can be especially important for automated methods that depend on real time monitoring and are sensitive to image degradations (e.g. flare detection). The refurbishing of legacy data is important for the study of long-term variability. The presented method provides an integral step for the usability of historic data sets, as demonstrated in Sect.~\ref{section:iti_restoration} for H$\alpha$ observations dating back to 1973. The approximation of missing observables, as demonstrated for LOS magnetograms in Sect.~\ref{section:iti_observables}, can provide additional information for solar monitoring and automated methods. We note that the magnetic polarity as provided by our model is ambiguous and should be interpreted in absolute value. This method can be applied in the same way for the approximation of different wavelength channels, that commonly differ between instruments.

%Considering the EUV filtergrams as input, the ITI results have a surprising similarity to real observations.
%A primary application of this method is the estimation of full-disk solar magnetograms and tracking of mage

%The approximation of magnetograms illustrates an extreme example, more reasonable could be the approximation of a similar EUV channe, maybe Ca II K from 304 AA

%This result supports the assumption that the magnetograms are derived from the EUV information, instead of only generating perceptually realistic images.

% We note that common full-reference quality metrics (e.g., MSE, RMSE) are not suitable, since a small misalignment can lead to large errors, and therefore blurred images usually result in better quality estimate than sharp images.

% discussion: no artificial flux emergence, no artifacts

